Rethinking The Uniformity Metric in Self-Supervised Learning

Uniformity plays an important role in evaluating learned representations, providing insights into self-supervised learning. In our quest for effective uniformity metrics, we pinpoint four principled properties that such metrics should possess. Namely, an effective uniformity metric should remain invariant to instance permutations and sample replications while accurately capturing feature redundancy and dimensional collapse. Surprisingly, we find that the uniformity metric proposed by \citet{Wang2020UnderstandingCR} fails to satisfy the majority of these properties. Specifically, their metric is sensitive to sample replications, and can not account for feature redundancy and dimensional collapse correctly. To overcome these limitations, we introduce a new uniformity metric based on the Wasserstein distance, which satisfies all the aforementioned properties. Integrating this new metric in existing self-supervised learning methods effectively mitigates dimensional collapse and consistently improves their performance on downstream tasks involving CIFAR-10 and CIFAR-100 datasets. Code is available at \url{https://github.com/statsle/WassersteinSSL}.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Self-supervised representation learning has become increasingly popular in machine learning community~\citep{Chen2020ASF,He2020MomentumCF,Caron2020UnsupervisedLO,Grill2020BootstrapYO,Chen2021ExploringSS,Zbontar2021BarlowTS}. It has been widely used in various tasks such as multimodality, object detection, and segmentation~\citep{Radford2021LearningTV,li2022supervision,Xie2021DetCoUC,Wang2021DenseCL,Yang2021InstanceLF,Zhao2021ContrastiveLF}. 
Aiming to learn transferable representations that are invariant to different augmentations, Siamese network~\citep{Hadsell2006DimensionalityRB} is widely used in self-supervised learning.
%a common practice of self-supervised learning is to maximize the similarity of representations obtained from different augmented versions of a sample by using a Siamese network~\citep{Hadsell2006DimensionalityRB}. 
However, a common issue with this approach is the existence of trivial constant solutions that all representations collapse to a constant point~\citep{Chen2021ExploringSS},  known as the collapse problem~\citep{Jing2021UnderstandingDC}. To avoid the collapse problem, many efforts have been made and well-known solutions can be summarized into three types: contrastive learning~\citep{Chen2020ASF,Caron2020UnsupervisedLO}, asymmetric model architecture~\citep{Grill2020BootstrapYO,Chen2021ExploringSS}, and redundancy reduction~\citep{Zbontar2021BarlowTS}. Nevertheless, these methods might still suffer from the dimensional collapse~\citep{hua2021feature} in which representations occupy a lower-dimensional subspace instead of the entire available embedding space~\citep{Jing2021UnderstandingDC}. As shown in Fig.~\ref{fig:singular value spectrum}, by conducting singular value spectrum analysis~\citep{Jing2021UnderstandingDC,Tian2021UnderstandingSL} on learned representations from various self-supervised models, we find that the dimensional collapse exists in most self-supervised models.

%We further provide empirical evidence can be found in Fig.~\ref{fig:singular value spectrum}. Therefore, to show the effectiveness of the aforementioned approaches, we need a quantifiable metric to measure the collapse degree of learned representations.

\begin{figure}[t]
\centering
\subfigure[Singular Value Spectrum]{ 
\label{fig:singular value spectrum}  	\includegraphics[width=0.37\textwidth]{figs/visualization/CIFAR_100_SVD.pdf}}
\hspace{-0.2cm}
\subfigure[Sensitivity to Collapse Level]{
\label{fig:sensitivity on collapse level}	\includegraphics[width=0.4\textwidth]{figs/analysis/DifferenceOnCollapseLevel.pdf}}
\vspace{-2mm}
\caption{(a) presents singular value spectrum analysis on 256-dimensional representations extracted from the CIFAR-100 dataset, indicating that the dimensional collapse exists in most self-supervised models. In (b), we empirically analyze the baseline uniformity metric $\mathcal{L_U}$~\citep{Wang2020UnderstandingCR} and our proposed metric $\mathcal{W}_{2}$ on the sensitivity to dimensional collapse level. Our proposed metric is capable of capturing salient sensitivity to collapse level, while $\mathcal{L_U}$ is insensitive to the dimensional collapse.
} 
\label{fig:introduction}
\vspace{-5mm}
\end{figure}


To better understand and analyze learned representations from various self-supervised models, how to achieve a quantifiable analysis of collapse degrees is an important research topic in the self-supervised learning community.
Towards this end, recent works~\citep{Arora2019ATA,Wang2020UnderstandingCR} propose to divide the loss function into alignment and uniformity terms. For instance, well-known objective functions such as InfoNCE~\citep{Oord2018RepresentationLW} and cross-correlation employed in Barlow Twins~\citep{Zbontar2021BarlowTS} could be divided into two terms. These uniformity terms could explain the degree of collapse to some extent, since they measure the variability of learned representations~\citep{Zbontar2021BarlowTS}. However, the calculation of these uniformity terms heavily relies on the choice of anchor-positive pair, making them hard to be used as general metrics.  \citet{Wang2020UnderstandingCR} introduce a formal uniformity metric via Radial Basis Function kernel~\citep{Cohn2006UniversallyOD}. Despite its usefulness %in analyzing collapse degree of representations, e.g., sentence embeddings
~\citep{Gao2021SimCSESC,Zhou2022DebiasedCL}, we theoretically demonstrate that the metric is insensitive to the dimensional collapse by checking on five well-designed  desirable properties (called `desiderata') of ideal uniformity metrics. Fig.~\ref{fig:sensitivity on collapse level} shows empirical evidence that the metric is insensitive to  dimensional collapse, as it is nearly in saturation when dimension level is  under 80\%.

In this paper, we focus on designing a new uniformity metric that could capture salient sensitivity to the dimensional collapse. Towards this end, we firstly introduce a finding that \textit{representation that obeys zero-mean isotropic Gaussian distribution is with the ideal uniformity}. %since its $\ell_2$-normalized form uniformly distributes on the surface of the unit hypersphere. 
Based on this finding, we use the Wasserstein distance between the distribution of learned representations and the ideal distribution as the metric of uniformity. %which can quantitatively analyze the dimensional collapse.}
%we fundamentally find that \textit{representation that obeys zero-mean isotropic Gaussian distribution  is  with the ideal uniformity} since its $\ell_2$-normalized form uniformly  distributes on the surface of the unit hypersphere. Based on the above finding, we use the Wasserstein distance between the distribution of learned representations and the ideal distribution as the metric of uniformity, which can  quantitatively analyze the dimensional collapse.
% we present a systematical analysis on collapse degree, and our work can be summarized into three steps. The first step is to propose a new uniformity metric that,  Towards this end, 
% Furthermore, to analyze the capacity on capturing  sensitivity to the dimensional collapse, we design five desirable constraints (desiderata) for ideal uniformity metrics. 
Our proposed metric is a superior uniformity metric to the existing one~\citep{Wang2020UnderstandingCR}, as the proposed uniformity metric can be theoretically demonstrated to satisfy all desiderata.
%By checking on five well-designed  desirable properties (called `desiderata') of uniformity, we theoretically demonstrate the proposed uniformity metric satisfies all desiderata while the existing one \citep{Wang2020UnderstandingCR} does not. 
Synthetic experiments also demonstrate the proposed  uniformity metric is capable of quantitatively distinguishing various dimensional collapse degrees while the existing one is insensitive.
%Furthermore, to facilitate comparison between our proposed uniformity metric and the existing one~\citep{Wang2020UnderstandingCR}, we design five desirable constraints (desiderata) for ideal uniformity metrics. Synthetic experiments also demonstrate the  proposed  uniformity metric is capable to deal with the dimensional collapse while the existing one is insensitive. 
Lastly, we apply our proposed uniformity metric in the practical scenarios, namely, imposing it as an auxiliary loss term for various existing self-supervised methods, which consistently improves the downstream performance.% in downstream tasks.


%To have a quantifiable analysis of collapse degree, we propose to use the Wasserstein distance between the distribution of learned representations and normal distribution as the uniformity metric, which could effective measures how uniformly learned representations distribute on surface of the unit hypersphere. 
%The underlying feasibility of the approach is that: \textit{if learned representations obey zero-mean isotropic gaussian distribution ($\m z \sim \mathcal{N}(\m 0, \m \sigma^2\m I)$), $\ell_2$-normalized forms ($\m z/\Vert \m z \Vert_2$) would distribute uniformly on the surface of the unit hypersphere space.} Smaller Wasserstein distance indicates larger uniformity and smaller collapse degree. 
%To facilitate further analysis on our proposed uniformity metric over other metrics in a mathematical manner, we also propose five desirable constraints that any reasonable uniformity metric should satisfy. Then, we theoretically and empirically demonstrate the superiority of our proposed uniformity metric against the metric proposed in~\citep{Wang2020UnderstandingCR}.

% The rest of the paper is organized as follows. We first review the background knowledge in Section~\ref{sec:background}, and then propose to use Wasserstein distance as the uniformity metric in Section~\ref{sec:method}. In Section~\ref{sec:criteria}, we present five formal constraints to evaluate the metric. Then we apply these constraints to compare our proposed metric with the metric proposed in~\citep{Wang2020UnderstandingCR} in Section~\ref{sec:theoretical_analysis}. \benyou{will check}
The contributions  are summarized as: 
(i) We  design five desirable properties that open a new perspective to rethink the ideal uniformity metrics; it shows
that the existing uniformity metric~\citep{Wang2020UnderstandingCR} is insensitive to the dimensional collapse, 
(ii) We propose a new uniformity metric that could capture salient sensitivity to the dimensional collapse;
and  (iii)  Our proposed uniformity metric can be applied as an auxiliary loss term in various self-supervised methods, which consistently improves the performance in downstream tasks.

\iffalse
The contributions of this work are as below: (i) \highlight{We introduce an interesting finding that \textit{representation that obeys zero-mean isotropic Gaussian distribution is with the ideal uniformity} metric, see Theorem \ref{proof:maximum uniformity}}; (ii) We design five desirable properties (Desiderata) for ideal uniformity; (iii) Based on Theorem \ref{proof:maximum uniformity}, we propose an new uniformity metric, which is theoretically and empirically proved to be superior to the existing one \citep{Wang2020UnderstandingCR}; and (iv) It could consistently improve the performance by using the proposed uniformity metric as an auxiliary loss in various self-supervised methods. \benyou{TBD}. %\benyou{@xianghong, please double check} 
\fi

==> sections/introduction_new.tex <==
\section{Introduction}
\label{sec:introduction}

%\paragraph{Introduction, Uniformity Perspective}


\iffalse
Self-supervised learning excels in acquiring transferable representations that remain invariant to  various augmentations, and it  has gained significant popularity within the machine learning community~\citep{Chen2020ASF,He2020MomentumCF,Caron2020UnsupervisedLO,Grill2020BootstrapYO,Zbontar2021BarlowTS}. This approach has found extensive application in diverse tasks, including multimodality learning, object detection, and segmentation~\citep{Radford2021LearningTV,li2022supervision,Xie2021DetCoUC,Wang2021DenseCL,Yang2021InstanceLF,Zhao2021ContrastiveLF}. The pursuit of  a deeper understanding of self-supervised learning stands as an important research avenue~\citep{Wang2021UnderstandingTB,Tian2022UnderstandingTR,Tian2022UnderstandingDC,Tian2021UnderstandingSL}. For instance, \citet{Arora2019ATA} and~\citet{Wang2020UnderstandingCR} propose to study self-supervised learning from the alignment and uniformity perspectives. In this paper, we focus on the uniformity perspective.
\fi



%\paragraph{Introducing SSL}

Self-supervised learning excels at acquiring invariant  representations %that exhibit invariance 
to various augmentations \citep{Chen2020ASF,He2020MomentumCF,Caron2020UnsupervisedLO,Grill2020BootstrapYO,Zbontar2021BarlowTS}. It has been outstandingly successful  across diverse domains, including multimodality learning, object detection, and segmentation \citep{Radford2021LearningTV,li2022supervision,Xie2021DetCoUC,Wang2021DenseCL,Yang2021InstanceLF,Zhao2021ContrastiveLF}. Ongoing research endeavors are dedicated to achieving a deeper understanding of self-supervised learning \citep{Arora2019ATA, Wang2021UnderstandingTB,Tian2022UnderstandingTR,Tian2022UnderstandingDC,Tian2021UnderstandingSL}.   \scomment{re-look at?}




\iffalse
\scolor{
Of particular significance is the work by \citet{Wang2020UnderstandingCR}, which takes {\it alignment} between positive pairs and {\it uniformity} of the whole representation space to quantitively measure the quality of learned representations.
}
\fi



%This paper focuses on the uniformity perspective. 

%identify two key properties related to contrastive learning—alignment and uniformity—and propose to use them to measure the quality of representations.
%For example, ~\citet{Wang2020UnderstandingCR} have proposed studying self-supervised learning from alignment and uniformity perspectives. In this paper, our focus is on the uniformity perspective.

\begin{wrapfigure}[11]{r}{0.46\textwidth}
\small
\vspace{-6mm}
\begin{center}
\includegraphics[width=0.44\textwidth]{figs/Collapse/ConstantCollapse_DimensionalCollapse.pdf}
\vspace{-2mm}
\caption{\small{The left figure presents constant collapse, and the right figure visualizes dimensional collapse.}}
\label{fig:two collapse types}
\end{center}
\end{wrapfigure} 


%\paragraph{Importance of Uniformity Perspective} 


\iffalse
Characterized by the variability of learned representations on the surface of a unit hypersphere, uniformity, as a supplement to alignment, plays an crucial role in evaluating the representation ability~\citep{Wang2020UnderstandingCR}. For example, Siamese network~\citep{Hadsell2006DimensionalityRB} suffers from a constant solution where all representations collapse into one single point~\citep{Chen2021ExploringSS}, as visualized in Fig.~\ref{fig:two collapse types}. This issue is commonly referred to as the ``collapse problem" \citep{Jing2021UnderstandingDC}. When such a collapse occurs, alignment is insufficient to measure representation capacity, since extremely small alignment between positive pairs (augmented image pairs from the same image) is with the worst performance. In other words, the invariant representations, generally regarded as the transferable representations that self-supervised learning approaches aim to learn, are with the worst representation ability. Therefore, it is appropriate to measure the capacity of learned representations by alignment solely.  To better evaluate learned representations, uniformity can be used as a new axis to make up the limitation of alignment, in particular in measuring collapse degree of representations. %uniformity is indispensable in evaluating learned representations.
\fi


%Uniformity characterizes the variability of learned representations on the unit hypersphere and plays a key role in measuring the quality of embeddings \citep{Wang2020UnderstandingCR}. 



%\paragraph{Alignment alone is a problem}

If the goal is to learn invariant embeddings only, simple Siamese networks \citep{Hadsell2006DimensionalityRB} are the natural tools as they concentrate on understanding the  variations and resemblances among images. However, collapsing solutions, where all outputs collapse  to one single point, exist for this model \citep{Chen2021ExploringSS}. This phenomenon is visualized in Figure \ref{fig:two collapse types}. 
When this occurs, the learned representations achieve the best alignment\footnote{Alignment means that two samples forming a positive pair should be mapped to nearby features, and thus be invariant to unneeded noise factors.} between positive pairs as they all collapse to one point, but fail to be informative in any downstream tasks. This indicates that {\it alignment} alone is not enough to measure the quality of learned representations. %We need uniformity as a new axis to measure the quality of representations, specifically the collapse degree of representations. 


 %As visualized in Figure \ref{fig:two collapse types}, a collapsing solution  refers to the case when all representations collapse to one single point \citep{Chen2021ExploringSS}. %This issue is commonly referred to as the ``collapse problem" \citep{Jing2021UnderstandingDC}.  


%\paragraph{Issue of Current Uniformity Metric}
\iffalse
To quantitatively measure the capacity of learned representations from the uniformity perspective, recent works~\citep{Arora2019ATA,Wang2020UnderstandingCR} propose to divide the loss function into alignment and uniformity terms. For instance, recent objective functions such as InfoNCE~\citep{Oord2018RepresentationLW} and cross-correlation employed in Barlow Twins~\citep{Zbontar2021BarlowTS} could be divided into two terms.  These uniformity terms could explain the degree of collapse to some extent, since they measure the variability of learned representations~\citep{Zbontar2021BarlowTS}. However, the calculation of these uniformity terms relies on the choice of anchor-positive pair, making them hard to be used as general metrics. 
Wang et al~\citep{Wang2020UnderstandingCR} further propose a formal definition of \emph{uniformity} metric via Radial Basis Function (RBF) kernel~\citep{Cohn2006UniversallyOD}. Despite its usefulness~\citep{Gao2021SimCSESC,Zhou2022DebiasedCL}, %in analyzing collapse degree of representations, e.g., sentence embeddings~\citep{Gao2021SimCSESC,Zhou2022DebiasedCL}, 
we theoretically and empirically demonstrate in later that the metric is insensitive to the dimensional collapse~\citep{hua2021feature}, where representations occupy a lower-dimensional subspace instead of the entire available embedding space~\citep{Jing2021UnderstandingDC}, as depicted in Fig.~\ref{fig:two collapse types}.
\fi


%\cite{Wang2020UnderstandingCR} argued that constrastive learning should prefer \cite
\citet{Wang2020UnderstandingCR} argued that feature embeddings should be roughly uniformly distributed on the unit hypersphere, preserving as much information of the data as possible. This property is referred to as {\it uniformity}. Indeed, the loss functions in many contrastive learning methods, such as InfoNCE \citep{Oord2018RepresentationLW} and Barlow Twins \citep{Zbontar2021BarlowTS}, can be decomposed into two terms, related to alignment and  uniformity respectively.  \cite{Wang2020UnderstandingCR}  formally proposed a \emph{uniformity} loss as the logarithm of the average pairwise Gaussian potential \citep{Cohn2006UniversallyOD}. Uniformity has since played an essential role in understanding contrastive learning and preventing constant collapse \citep{Arora2019ATA,Wang2020UnderstandingCR}.  



\iffalse
In this paper, we introduce a novel perspective and take a step further to rethink the uniformity measure within self-supervised learning setting. First, we propose four well-designed desirable properties (called `desiderata') of ideal uniformity metrics. Then, we propose to design a new uniformity metric that could capture salient sensitivity to the dimensional collapse. Towards this end, we firstly introduce a finding that \textit{representation that obeys zero-mean isotropic Gaussian distribution is with the ideal uniformity}. Based on this finding, we use the Wasserstein distance between the distribution of learned representations and the ideal distribution as the metric of uniformity. Our proposed metric is a superior uniformity metric to the existing one~\citep{Wang2020UnderstandingCR}, as the proposed uniformity metric can be theoretically demonstrated to satisfy all desiderata.
Synthetic experiments also demonstrate the proposed  uniformity metric is capable of quantitatively distinguishing various dimensional collapse degrees while the existing one is insensitive.
Lastly, we apply our proposed uniformity metric in the practical scenarios, namely, imposing it as an auxiliary loss term for various existing self-supervised methods, which consistently improves the downstream performance.
\fi 

Despite its success in preventing constant collapse, we show in this paper, both theoretically and empirically, that the metric by \cite{Wang2020UnderstandingCR} is insensitive to the dimensional collapse~\citep{hua2021feature}, where representations occupy a lower-dimensional subspace instead of the entire  embedding space~\citep{Jing2021UnderstandingDC}; see Figure~\ref{fig:two collapse types}. Towards addressing this problem, %we take a step further to rethink what an ideal  uniformity measure should obey. Specifically, 
we propose four properties, referred to as desiderata, that an  ideal uniformity metric should follow. We then propose  a new uniformity metric that is sensitive to dimensional collapse. 
Our proposed uniformity metric satisfy all desiderata while that by \cite{Wang2020UnderstandingCR} does not. 
Synthetic experiments  demonstrate that the proposed  uniformity metric is sensitive to various dimensional collapse degrees while the one by \cite{Wang2020UnderstandingCR}. 
Using the proposed uniformity metric as an auxiliary loss within existing self-supervised learning methods consistently improves their performance in downstream tasks. 


% Towards this end, we firstly introduce a finding that \textit{representation that obeys zero-mean isotropic Gaussian distribution is with the ideal uniformity}. Based on this finding, we use the Wasserstein distance between the distribution of learned representations and the ideal distribution as the metric of uniformity. 


%Lastly, we apply our proposed uniformity metric in the practical scenarios, namely, imposing it as an auxiliary loss term for various existing self-supervised methods, which consistently improves the downstream performance.
%When applying the proposed uniformity metric instead of the o




%is a superior uniformity metric to the existing one~\citep{Wang2020UnderstandingCR}, as the proposed uniformity metric can be theoretically demonstrated to satisfy all desiderata.


% theoretically and empirically show 

%Radial Basis Function (RBF) kernel~\citep{Cohn2006UniversallyOD}.

%Despite its usefulness~\citep{Gao2021SimCSESC,Zhou2022DebiasedCL}, %in analyzing collapse degree of representations, e.g., sentence embeddings~\citep{Gao2021SimCSESC,Zhou2022DebiasedCL}, 
%we theoretically and empirically demonstrate in later that the metric is insensitive to the dimensional collapse~\citep{hua2021feature}, where representations occupy a lower-dimensional subspace instead of the entire available embedding space~\citep{Jing2021UnderstandingDC}, as depicted in Fig.~\ref{fig:two collapse types}.


%takes {\it alignment} between positive pairs and {\it uniformity} of the whole representation space to quantitively measure the quality of learned representations.



%\paragraph{Summary of Contributions}

%The contributions  are summarized as:
%We summarize our main contributions as follows. 
%(i) We  design five desiderata that provide a new perspective to rethink the ideal uniformity metrics; it shows
%that the existing uniformity metric~\citep{Wang2020UnderstandingCR} is insensitive to the dimensional collapse, 
%(ii) We propose a new uniformity metric that could capture salient sensitivity to the dimensional collapse;
%and  (iii)  Our proposed uniformity metric can be applied as an auxiliary loss term in various self-supervised methods, which consistently improves the performance in downstream tasks.

Our main contributions can be summarized as follows.
(i) We introduce four desiderata that offer a fresh perspective on designing the ideal uniformity metrics. The existing uniformity metric \citep{Wang2020UnderstandingCR}   does not satisfy all desiderata, and our empirical studies  reveal that it is  insensitive to dimensional collapse.
(ii) We put forth a novel uniformity metric designed to effectively capture sensitivity to dimensional collapse.
(iii) Our newly proposed uniformity metric can be seamlessly integrated as an auxiliary loss in a variety of self-supervised methods, consistently enhancing their performance in downstream tasks.



\iffalse
\paragraph{Related Work}
\scolor{
We briefly review related work. related work on contrastive learning. 
}
\fi
